Detecting and Handling Flash-Crowd Events on Cloud Environments

Cloud computing is a highly scalable computing paradigm where resources are delivered to users on demand via Internet. There are several areas that can benefit from cloud computing and one in special is gaining much attention: the flash-crowd handling. Flash-crowd events happen when servers are unable to handle the volume of requests for a specific content (or a set of contents) that actually reach it, thus causing some requests to be denied. For the handling of flash-crowd events in Web applications, clouds can offer elastic computing and storage capacity during these events in order to process all requests. However, it is important that flash-crowd events are quickly detected and the amount of resources to be instantiated during flash crowds is correctly estimated. In this paper, a new mechanism for detection of flash crowds based on concepts of entropy and total correlation is proposed. Moreover, the Flash-Crowd Handling Problem (FCHP) is precisely defined and formulated as an integer programming problem. A new algorithm for solving it, named FCHP-ILS, is also proposed. With FCHP-ILS the Web provider is able to replicate contents in the available resources and define the types and amount of resources to instantiate in the cloud during a flash-crowd event. Finally we present a case study, based on a synthetic dataset representing flash-crowd events in small scenarios aiming at comparing the proposed approach with de facto standard Amazon's Auto Scaling mechanism.

==> flashcrowd.tex <==
\section{Traces of Flash Crowds}
\label{sec:background}
	
	Flash crowds can be characterized by several factors, such as duration, growth rate, and locality. A flash-crowd event at a web site has three main phases \cite{artigo-2}: a \textit{ramp-up} phase, a \textit{sustained-traffic} phase, and a \textit{ramp-down} phase. Starting at a traffic pattern that is considered normal, during the ramp-up phase traffic rises significantly for a small number of contents and can stay high for some time, depending on the kind of flash crowd. In the ramp-down phase the number of accesses gradually decreases until traffic becomes once again normal. Due to the difficulty in obtaining real traces to evaluate the method for handling flash crowds, a generator of synthetic flash crowds was developed. This generator can produce several kinds of traces by modeling flash crowd's main phases and taking into account some of the characteristics of real flash crowds. It is based on sampling from a variety of beta distributions, as discussed next.
		
	Assume any given content and let $X_t$ be a discrete random variable representing the number of accesses to that content at time $t$. Assume further that $X_t$ takes values from the domain $[0,U]$ for some integer $U>0$. Our goal is to devise a probability mass function on the integers in $[0,U]$ such that sampling from the corresponding distribution can generate a number of accesses to the content in question for any time $t$. Although our random variable is not continuous, the use of a bounded support such as $[0,U]$ immediately suggests the beta density function, whose support is $[0,1]$. What we do is to adopt this function nevertheless, noting that every sample is to be rounded off to an integer after being scaled up by the factor $U$. The beta density function to be used in sampling a value $x$ for $X_t$, henceforth denoted by $p_t(x)$, is given by
$$
p_t(x)=\frac{x^{\alpha_t-1}(1-x)^{\beta_t-1}}{\Gamma(\alpha_t)\Gamma(\beta_t)/\Gamma(\alpha_t+\beta_t)},
$$
where $\alpha_t$ and $\beta_t$ are both positive and control the function's shape through its mean, $\alpha_t/(\alpha_t+\beta_t)$, and variance, $\alpha_t\beta_t/(\alpha_t+\beta_t)^2(\alpha_t+\beta_t+1)$.

	This shape parameterization is convenient for the generation of flash crowd accesses, particularly during the ramp-up and ramp-down phases. To see this, consider two instants $t_0<t_1$ and the modeling of the ramp-up phase of a flash crowd between $t=t_0$ and $t=t_1$. We first choose $\alpha_{t_0}\ll\beta_{t_0}$, so that $X_{t_0}$, the number of accesses right before the ramp-up phase, has a low mean and a relatively low variance. Likewise, in order to get high values for $X_{t_1}$, that is, right past the ramp-up phase, we choose $\alpha_{t_1}\gg\beta_{t_1}$. The latter can be achieved, for example, by setting $\alpha_{t_1}=\beta_{t_0}$ and $\beta_{t_1}=\alpha_{t_0}$, which implies a high mean and also both $\alpha_{t_1}+\beta_{t_1}=\alpha_{t_0}+\beta_{t_0}$ and $\alpha_{t_1}\beta_{t_1}=\alpha_{t_0}\beta_{t_0}$, thence the same relatively low variance as before. This particular choice for $\alpha_{t_1}$ and $\beta_{t_1}$ is therefore quite handy, because it immediately allows all intermediate values of $t$ (i.e., the ramp-up phase itself) to be handled easily: We simply let
$$
\alpha_t=y_t\alpha_{t_0}+(1-y_t)\beta_{t_0}
$$
with $0\le y_t\le 1$ and
$$
\beta_t=\alpha_{t_0}+\beta_{t_0}-\alpha_t.
$$
That is, both $\alpha_t$ and $\beta_t$ are convex combinations of $\alpha_{t_0}$ and $\beta_{t_0}$. Setting $y_t=1$ recovers $p_{t_0}(x)$; setting $y_t=0$ recovers $p_{t_1}(x)$.

	As for sampling $X_t$ during the ramp-up phase itself, all that is left to do is to decide the rate at which $y_t$ is decreased from $1$ at $t=t_0$ to $0$ at $t=t_1$. Here we let $y_t$ decrease in such a way that $1-y_t$ increases exponentially. That is,
$$
y_t=\frac{e^{\gamma(t_1-t_0)}-e^{\gamma(t-t_0)}}{e^{\gamma(t_1-t_0)}-1}
$$
for some $\gamma>0$, which implies a ``generally convex'' growth pattern in the number of accesses. The number of accesses for any time prior to the ramp-up phase can be sampled as $X_{t_0}$. For times in the sustained-traffic phase, the number of accesses can be sampled as $X_{t_1}$.

	Modeling instead a ramp-down phase from $t_0$ to $t_1$ can be done essentially along the same lines. We simply let both $\alpha_t$ and $\beta_t$ be given as above and increase $y_t$ from $0$ at $t=t_0$ to $1$ at $t=t_1$. We do this in such a way that $y_t$ increases exponentially, that is,
$$
y_t=\frac{e^{\gamma(t-t_0)}-1}{e^{\gamma(t_1-t_0)}-1}
$$
with $\gamma>0$, which promotes a ``generally concave'' decay pattern in the number of accesses. The number of accesses for any time past the ramp-down phase can be sampled as $X_{t_1}$.



==> formulation.tex <==
\subsection{Mathematical Formulation}
\label{sec:formulation}

In order to describe formulation FCHP-IP, we need to extend the notation defined in Section \ref{sec:model}. Let $S=S_p \cup S_e$ be the set of all servers (virtual or physical), where $S_p$ and $S_e$ are defined as the set of Web application servers and the set of servers available for hire in the cloud, respectively. We also consider a set of requests $R$ to be attended and a set of  contents $C$ offered by the Web application in a period of time $t\in T = \{T_1,\dots,T_{f}\}$. Each request $i \in R$ requires a content and each content $k \in C$  has a size $L_k$. Each server $j \in S$ has a storage capacity $AS_{j}$ and a maximal bandwidth $MB_{j}$ and each server $j \in S_e$ also has a financial cost $f_j$. Similarly, each content $k \in C$ has a start time $B_{k}$ (\textit{i.e.} the period that content $k$ is submitted in the application) and an origin server $O_{k}$. Moreover, each request $i \in R$ requires a content $g(i)$ and we denote as $D_{it}$, the demand of request $i \in R$ in period $t \in T$. Finally, we define $BX$ as the average bandwidth of the clients. 

Now we can restate the FCHP as the problem of copying replicas of contents on the servers and hiring new cloud servers in order to handle the requests during the flash crowd, respecting the available storage and bandwidth and trying to minimize the cost function defined by four sums of time: (i) the time cost $c_{i}$ to handle request $i \in R$, defined by $\sum_{i\in R}  \sum_{j \in S} \sum_{t\in T} c_{i}x_{ijt}$, where the binary variable $x_{ijt}$ indicates if the request $i$ is attended by server $j$ in period $t$, (ii) the sum of backlogging time penalty $p_{it}$ (\textit{i.e.} the penalty to postpone the attendance of request $i$ that arrived in period $t$), defined by $\sum_{i \in R} \sum_{t \in T} p_{it}b_{it}$, where $b_{it}$ indicates the postponed amount of request $i$ in period $t$, (iii) the sum of time cost $h_{k}$ to copy the content $k$, defined by $\sum_{k \in C} \sum_{j \in S} \sum_{l \in S} \sum_{t \in T} h_{k}w_{kjlt}$, where the binary variable $w_{kjlt}$ indicates if the content $k$ is copied from server $j$ to server $l$ in period $t$, and (iv) the sum of financial cost $f_j$ to hire the server $j$ in period $t$, defined by $ \sum_{j \in S} \sum_{t \in T} f_{j}z_{jt} \frac{1}{M} $, where the binary variable $z_{jt}$ indicates if the server $j$ is hired in period $t$ and $M=\max\{c_i,p_{it}b_{it},h_k,f_j\}$ $\forall i \in R, t \in T, k \in C $ and $j \in S_e$. Note that the fourth sum can not be greater than any other cost in the previous sums. So, this last sum works as a tiebreaker for solutions with the same time cost to obtain the one with the minimal financial cost. 
%
Furthermore, we also define other three binary variables: $y_{kjt}$ that indicates if content $k \in C$ is replicated on server $j \in S$ in period $t \in T$; $s_{iojt}$ that indicates if the demand of request $i \in R$ of period $o \in T$ (i.e. $D_{io}$) is attended by server $j \in S$ in period $t \in T$. 
%
Note that the expression $ \sum_{o=1}^{t} ( s_{iojt}D_{io} )$ is equivalent to the amount of demand attended of request $i$ in server $j$ on period $t$.
%
Finally, variable $z_{jt}$ indicates if server $j \in S_e$ is hired in period $\alpha \in \overline{T}=\{\overline{T_1},\ldots,\overline{T_f}\}$. Note that the time scale $\overline{T}$ can have a granularity greater than $T$ due to the minimal hiring period offer by the cloud provider. 
We also define two constants, $tr$ and $tp$, representing the number of periods that a replication takes to be available and the number of periods that a hired server takes to be available, respectively.
%
The FCHP can be formulated as the mixed integer programming problem described in Figure \ref{modelo}.
%The FCHP can be formulated as the following mixed integer programming problem:

\begin{figure*}

%\begin{table*}[!htb]
\begin{align}
\mathrm{minimize\ } &  \sum_{i\in R}  \sum_{j \in S} \sum_{t\in T} c_{i}x_{ijt} + \sum_{r \in R} \sum_{t \in T} p_{it}b_{it} + \sum_{k \in C} \sum_{j \in S} \sum_{l \in S}\sum_{t \in T} h_{k}w_{kjlt} + \sum_{j \in S} \sum_{t \in T} f_{j}z_{jt} \frac{1}{M}& \label{fo4}\\
\mathrm{subject\ to\ } & &\nonumber\\
                 & \sum_{j \in S} \Big(  \sum_{o=1}^{t} ( s_{iojt}D_{io} ) \Big)  = D_{it}+ (b_{i(t-1)}-b_{it}), & \forall i \in R,  \forall t \in [B_{g(i)},T_f] \label{r1}\\
                 & \sum_{i \in R} \Big(  \sum_{o=1}^{t} ( s_{iojt}D_{io} ) \Big) \leqslant MB_{j},            & \forall j \in S,  \forall t \in T  \label{r2}\\
                 & \sum_{j \in S} \Big(  \sum_{o=1}^{t} ( s_{iojt}D_{io} ) \Big) \leqslant BX,                & \forall i \in R, \forall t \in T  \label{r3}\\
                 & \sum_{j \in S} \sum_{t \in T}\Big(  \sum_{o=1}^{t} ( s_{iojt}D_{io} ) \Big) = L_{g(i)},    & \forall i \in R  \label{r4}\\
                 & \sum_{o=1}^{t} ( s_{iojt}D_{io} ) \leqslant x_{ijt}L_{g(i)},                               & \forall i \in R, \forall j \in S, \forall t \in T \label{r4-1}\\
                 & y_{g(i)jt} \geqslant x_{ijt},                                                              & \forall i \in R, \forall j \in S, \forall t \in T  \label{r5}\\
                 & y_{kO_{k}B_{k}} = 1,                                                                       &\forall k \in C \label{r6}\\
                 & \sum_{\substack{t=1\ldots\\(B_k)}} \sum_{j \in S} y_{kjt} = 0 ,                            &\forall k \in C \label{r7}\\
                 & \sum_{\substack{j \in S\\j \neq O_k}} y_{kjB_k} = 0 ,                                      & \forall k \in C \label{r8}\\
                 & \sum_{\substack{t=1\ldots\\(B_k)}} w_{kjlt} = 0 ,                                          & \forall k \in C, \forall j \in S, \forall l \in S \label{r9}\\
                 & y_{kj(t+tr)} \leqslant \sum_{l \in S}w_{kjlt},                                             & \forall k \in C, \forall j \in S,   \forall t \in [B_k,T_f] \label{r10} \\ 
                 & y_{kjt} \geqslant w_{kljt},                                                                & \forall k \in C, \forall j \in S, \forall l \in S,  \forall t \in [B_k,T_f]\label{r11}\\ 
                 & \sum_{k \in C} L_{k}y_{kjt} \leqslant AS_{j},                                              & \forall j \in S, \forall t \in T\label{r12}\\
                 & x_{ijt} \leq z_{j\alpha} ,                                                                 & \forall i\in R, \forall j \in S_e, \forall (t-tp) \in [\alpha-1,\alpha], \alpha \in \overline{T}\label{r13}\\
                 & x_{ijt} \in \{0,1\},       																& \forall i \in R, \forall j \in S,  \forall t \in T\label{r14-1}\\
                 & b_{it} \geqslant 0,																        & \forall i \in R, \forall j \in S,  \forall t \in T\label{r14-2}\\
                 & s_{iojt} \in \{0,1\},     															    & \forall i \in R, \forall j \in S,  \forall t,o \in T\label{r14-3}\\
                 & y_{kjt} \in \{0,1\},									                                    & \forall k \in C, \forall j \in S,  \forall t \in T\label{r15}\\
                 & z_{jt} \in \{0,1\},									                                    & \forall k \in C, \forall j \in S,  \forall t \in T\label{r15}\\
                 & w_{ijlt} \in \{0,1\},                                                                      &\forall j,l \in S,  \forall k \in C, \forall t \in T\label{r17}
\end{align}
%
\caption{FCHP-IP formulation.}
\label{modelo}
%\end{table*}
\end{figure*}
%
%where $tr$ and $tp$ are the number of periods that a replication takes to be available and the number of periods that a hired server takes to be available, respectively.

The objective function (\ref{fo4}) minimizes the operational time costs, backlog and financial cost. 
%
Constraints (\ref{r1}) relate the demand attended of request $i \in R$ in period $t \in [B_{g(i)},T_f]$ (i.e. left-hand side of the equation) with the postponed and inherited backlog (i.e. $b_{it}$ and $b_{i(t-1)}$ respectively). 
%
Servers bandwidth are controlled by constraints (\ref{r2}). Constraints (\ref{r3}) prevent that a client receive more than it can bear. Constraints (\ref{r4}) guarantee that every request is fully handled. 
%
Constraints (\ref{r4-1}) relate the variables $s_{iojt}$ and $x_{ijt}$. Note that, if $s_{iojt}=1$ for any $o \in T$, then we should impose $x_{ijt}=1$.
%
Constraints (\ref{r5}) rule that a request must be handled by a server that has a replica of the desired content. Constraints (\ref{r6}), (\ref{r7}), (\ref{r8}) and (\ref{r9}) control the number of replicas of active contents and make sure that only the origin server has a replica of the content on the submission period. Constraints (\ref{r10}) guarantee that all replications create a new replica. Constraints (\ref{r11}) make sure that a replication occurs from a server that has the content. The servers storage capacity are controlled by constraints (\ref{r12}). Constraints (\ref{r13}) impose that a request must be handled by a hired server. The remaining constraints are the integrality and non-negativity constraints.




==> results.tex <==
\section{Experimental Results}
\label{sec:result}

In this section, we present the results for two accomplished tests. The fist one is a  comparison between the FCHP-IP mathematical formulation and the FCHP-ILS heuristic. The second is a  comparison between the combination of FCHP-ILS heuristic and FCD mechanism and the combination of  Amazon’s Auto Scaling and Load Balancing mechanisms \cite{AS,ELB}  executed in two real small-scale scenarios.

\subsection{Comparing FCHP-IP and FCHP-ILS}
	 We evaluate FCHP-ILS, in terms of  quality of solution and execution time,  by comparing it with the solutions given by the formulation FCHP-IP when solved with the CPLEX $12.5.1$ \cite{cplex}. Those tests were run  in a computer with a processor Intel Core i7-3820 3.60GHz  and  a 32Gb memory running Ubuntu $12.04$. The  FCHP-ILS was implemented in the Programming language C/C++, gcc version $4.6.3$.
	
	 Those programs were run over a set of instances created from a  real trace obtained from the 1998 World Cup site \cite{copa98}.  Because this trace presents a huge number of requests, the total time of the trace was discretized in hours and only the requests for the ten most accessed contents in each interval of time were considered. Thus, instances with reduced size, but still presenting flash-crowd events, were created. Remark that the original instance could not be solved in a reasonable time by the CPLEX. 

	 %The six created instances have, in average, $81.7$ contents and $2228.7$ requests. The first three instances contain requests presented in a period of $12$ hours and the last three contain requests presented in a period of $24$ hours.
	 Table \ref{Instance} presents for each of the twelve created instances, the  associated number of contents, requests and number of periods (hours). The last two instances were created by the synthetic trace generator and used for the real experiments, described in the next section.
	
\begin{table}[htp]
\small
\setlength{\tabcolsep}{3mm}
\caption{Instance description}
\begin{center}
\setlength{\tabcolsep}{0.6mm}
\begin{tabular}{|c|r|r|r|}
\hline 
Instance & \# of Contents  & \# of Requests & Periods (hours) \\
%\cline{8-16} 
\hline
1	&	44	&	1798		&	12		\\
2	&	60	&	1696		&	12	    \\
3	&	88	&	983	    	&	12		\\
4	&	52	&	3546		&	24		\\
5	&	96	&	3427		&	24		\\
6	&	150	&	1922		&	24		\\
7   &   47  &   4327	    &   36      \\
8   &   83  &   4073        &   36      \\
9   &   99  &   1676        &   36      \\
10   &  69  &   7110 		&   48      \\
11   &   3  &   105         &   60      \\
12   &   4  &   186         &   60      \\
\hline
\end{tabular}
\end{center}
\label{Instance}
\end{table}
	
Table \ref{teorico} shows the results obtained by FCHP-IP and FCHP-ILS. The first column identifies the instance. The following six columns present the results obtained by FCHP-IP: number of hired  on demand servers, the total cost, the attendance cost, replication cost, backlog cost and the execution time to obtain the optimum solution. Following, the next columns present the same results of FCHP-ILS. Finally, the last column, shows the gap between the solutions given by FCHP-ILS and FCHP-IP. The  values shown for FCHP-ILS are averages of three executions, where  $3$, $7$ and $1$ were used for the number of iterations, the number of perturbations and the value of $d$ ({\bf $d-$Delay} neighbourhood), respectively. 


\begin{table*}[htp]
\small
\caption{Results of FCHP-ILS Metaheuristic and FCHP-IP Mathematical Formulation using CPLEX}
\begin{center}
\setlength{\tabcolsep}{1.1mm}
\begin{tabular}{|c|crrrcr|crrrcr|c|}
\hline 
\multirow{3}{1cm}{Instance} & \multicolumn{6}{|c|}{FCHP-IP} & \multicolumn{6}{|c|}{FCHP-ILS} & \multirow{3}{1cm}{Gap(\%)}\\
\cline{2-13}
 & Serv & \multicolumn{4}{|c|}{Time Cost} & & Serv & \multicolumn{4}{|c|}{Time Cost} & & \\
 &  OD & \multicolumn{1}{|c}{Total} & Attend & Repli & \multicolumn{1}{c|}{Back} & Time & OD & \multicolumn{1}{|c}{Total} & Attend & Repli & \multicolumn{1}{c|}{Back} & Time &\\
\hline 
1	&	14	&	1726.9	&	1639.6	&	87.3	&	0	&	134.6	&	7	&	2647.0	&	2486.3	&	160.8	&	0	&	93.7	&	53.3	\\
2	&	8	&	1993.6	&	1869.2	&	124.4	&	0	&	174.9	&	6	&	2139.6	&	1979.2	&	160.4	&	0	&	57.8	&	7.3	\\
3	&	8	&	607.4	&	446.6	&	160.8	&	0	&	44.2	&	2	&	749.4	&	573.3	&	176.1	&	0	&	73.8	&	23.4	\\
4	&	8	&	3512.8	&	3349.2	&	163.6	&	0	&	546.5	&	15	&	5570.4	&	5242.5	&	327.8	&	0	&	359.1	&	58.6	\\
5	&	26	&	2065.3	&	1775.4	&	289.9	&	0	&	230.1	&	5	&	2390.8	&	2065.4	&	325.4	&	0	&	168.5	&	15.8	\\
6	&	55	&	7167.0	&	6664.4	&	502.6	&	0	&	36619.4	&	9	&	8355.6	&	7604.4	&	751.2	&	0	&	185.7	&	16.6	\\
7	&	12	&	4991.3	&	4785.4	&	205.9	&	0	&	781.4	&	19	&	7914.9	&	7505.4	&	409.5	&	0	&	319.6	&	58.6	\\
8	&	10	&	3721.1	&	3344.6	&	376.5	&	0	&	610.2	&	15	&	5616.8	&	5084.6	&	532.2	&	0	&	230.4	&	50.9	\\
9	&	19	&	1179.1	&	750.4	&	428.7	&	0	&	280.2	&	8	&	1622.2	&	1040.4	&	581.8	&	0	&	79.7	&	37.6	\\
10*	&	43	&	7586.3	&	7202.0	&	384.3	&	0	&	2483.8	&	26	&	11763.0	&	11087.0	&	681.7	&	0	&	1308.6	&	55.1	\\
11*	&	440	&	28451.7	&	21957.4	&	6494.3	&	0	&	7388.8	&	123	&	28764.8	&	21957.4	&	6807.4	&	0	&	967.5	&	1.1	\\
12*	&	239	&	41228.2	&	32208.9	&	9019.3	&	0	&	14382.2	&	282	&	42036.2	&	32208.9	&	9827.3	&	0	&	6564.4	&	2.0	\\

%1	&	7	&	1689.0	&	1639.6	&	49.4	&	0	&	222.3	&	6.3	&	2093.7	&	1942.9	&	150.8	&	0	&	67.8	&	24.0	\\
%2	&	6	&	1937.4	&	1869.2	&	68.2	&	0	&	244.8	&	6	&	2153.5	&	1989.2	&	164.3	&	0	&	60.6	&	11.2	\\
%3	&	0	&	520.4	&	446.6	&	73.8	&	0	&	61.5	&	2	&	792.8	&	613.3	&	179.5	&	0	&	72.4	&	52.3	\\
%4	&	40	&	3441.9	&	3349.2	&	92.7	&	0	&	625.1	&	15.3	&	5620.4	&	5295.9	&	324.5	&	0	&	390.0	&	63.3	\\
%5	&	4	&	1910.8	&	1775.4	&	135.4	&	0	&	391.1	&	5	&	2602.3	&	2255.4	&	346.9	&	0	&	168.7	&	36.2	\\
%6	&	51	&	6907.3	&	6664.4	&	242.9	&	0	&	18875.6	&	9	&	8538.3	&	7787.7	&	750.5	&	0	&	203.4	&	23.6	\\
%
%
%
%7   &   440 & 28451.7 & 21957.4 & 6494.3 &  0 &  7388.84 & 123 & 28764.8 & 21957.4 & 6807.4 & 0 &  967.49 & 1.1\\
%8   &   239 & 41228.2 & 32208.9 & 9019.3 &  0 &  14382.2 & 282 & 42036.2 & 32208.9 & 9827.3 & 0 &  6564.41& 2.0 \\
\hline
Average	&		&		&		&		&		&	5306.4 	&		&		&		&		&		&	867.4 	&	31.7	\\
\hline 
\end{tabular}
\end{center}
\label{teorico}
\end{table*}
	

	In this table, we can observe a high gap for some instances. This is due to the difficult of the considered problem. The FCHP problem extends the Replica Placement Problem (RPP), which belongs to the NP-hard class \cite{aioffi05}. For small instances of the problem,  FCHP-ILS   takes a long time to find good solutions. However, as the input data increases, the FCHP-IP is not capable of proving the optimality of the solution in a reasonable time. Moreover,  FCHP-IP needs a higher memory capacity to solve bigger instances.  The results for instances $6$, $11$ and $12$ show that FCHP-ILS is more suitable in those cases, when  the gap and the execution time were reduced when compared with the averages results. Furthermore, in the last three instances, the CPLEX could not prove the optimality of the solution due to lack of memory. Remark that the two last instances were used in the real experiments.
	
\subsection{Comparing FCHP-ILS and Auto Scaling in real scenarios}	
		
	In order to analyze the performance of FCHP-ILS combined with the FCD as a single approach for  detecting and handling flash crowd in a  commercial cloud, we executed the procediments in a small scenario and compared with the mechanism provided by the  popular  Auto Scaling and Load Balancing of the Amazon.
	We used a synthetic trace generator of flash-crowd events %,  described in Section \ref{sec:background}, 
	to generate the  clients'  requests.  The  Web application was developed using Apache Tomcat $6.0$ \cite{tomcat}.
%	
	%In the first scenario, the Web application offers  three different contents  with  the following sizes: $1.9$, $1.5$ and $0.9$ Gbytes. The \textit{ramp-up phase} occurs between $1140$ and $1740$ seconds, the \textit{sustained traffic phase} from $1800$ to $1860$ seconds,  and the \textit{ramp-down phase} in the interval from $1920$ to $2460$ seconds, as shown in  Figure \ref{fc-figure}(a). Figure \ref{fc-figure}(b) presents the total number of requests  that were not attended  yet in  each second. 
	
	We also consider that the Web application offers four different contents  with  the following sizes: $0.8$, $1.0$, $1.5$ and $2.0$ Gbytes. In this scenario there are two flash-crowd events. For the first flash crowd, the \textit{ramp-up phase} occurs between $540$ and $1140$ seconds, the \textit{sustained traffic phase} from $1200$ to $1320$ seconds,  and the \textit{ramp-down phase} in the interval from $1380$ to $1860$ seconds. For the second one,  the \textit{ramp-up phase} occurs between $1500$ and $2100$ seconds, the \textit{sustained traffic phase} from $2160$ to $2220$ seconds,  and the \textit{ramp-down phase} in the interval from $2280$ to $2820$ seconds. The number of new requests and requests to be attended per second for this scenario are shown in Figure \ref{fc2-figure}(a). The Figure \ref{fc2-figure}(b) presents the value of the total correlation. Note that even in this small scenario, where the number of accesses is small and sparse, the total correlation can precisely detect the flash-crowd event.
	%The Figure \ref{fc2-figure}(b) presents the values of the joint entropy and total correlation. Note that differently from the 1998 World Cup case illustrated in Section \ref{sec:detection}, where both joint entropy and total correlation indicate the beginning and the end of the flash crowd, in this small scenario just the total correlation can detect precisely the flash crowd. This is related to the size of the tested scenario, where the number of accesses is small and sparse, resulting in a large variation of the entropies. Thus, this fact reinforces the choice of the total correlation as the main information to detect the flash crowd events.
	% This occurs due to the size and sparsity of this scenario, where the small number of accesses makes the entropies vary.
		
	In this test, the servers' bandwidth is  $10$ Mbytes/s while  the clients' bandwidth  is $1$ Mbytes/s  bandwidth  in average. The contents of $0.8$ and $1.0$ Gbytes was the only involved in the flash crowd. Note that the Web application starts by using two virtual machines of type \textit{m3.large}  of the Amazon.
	
	The main objective to create and execute this scenario was to analyze how these two approaches, Auto Scaling and  FCHP-ILS,  behave in a flash-crowd event with two distinct contents at overlapping periods of time. 

	%To have a fair comparison, in both approaches, the flash crowd was detected in the same time and the Web application started by using two virtual machines of type \textit{m3.large}  of the Amazon, each one containing all the contents.	
	

\begin{figure*}[ht]
\centering
\begin{center}
\begin{tabular}{c c}
\includegraphics[scale=0.5]{fig/acessos_real_2_seg.pdf} & \includegraphics[scale=0.5]{fig/Todos_med2_cxy.pdf} \\
(a) & (b) \\
\end{tabular}
\end{center}
\caption{(a) New requests and requests to be attended per second. (b) Total correlation for the tested scenario.}
\label{fc2-figure}
%\setlength{\belowcaptionskip}{-0.2cm}
\end{figure*}	

%\begin{figure}
%\centering
%\includegraphics[scale=0.4]{fig/acessos_seg.pdf}	
%\caption{Flash crowd access.}
%\label{fc-figure}
%\end{figure}		

	The Auto Scaling was configured to allocate new virtual machines (Web servers) % in the beginning of the flash crowd. 
	when the servers bandwidth usage exceeds 70\%.
	Note that, during a flash crowd, the solution provided by Auto Scaling allocates virtual machines based on a static virtual image that must contain all contents of the Web application.
	%Note that, during a flash crowd,  the solution provided by   the  Auto Scaling  allocates virtual machines exactly equal to the original used ones, that must contain all contents of the Web application. 
	 So it continued to use  \textit{m3.large} virtual machines,  which have  enough capacity to store the three contents. The  Load Balancing service is employed to evenly distribute the client's requests among the used  servers. 
	
	In our approach, requests are treated by a machine that has a similar role  of the one which executes the Auto Scaling and  Load Balancing service. It is responsible for directing the received requests to the virtual machines; when a flash crowd  occurs,  executing   FCHP-ILS;   and,  in accordance with the results given by FCHP-ILS, replicating contents or allocating  new virtual machines. Remark, however, that in our approach the new  allocated virtual machines can be different from the originally allocated ones. It allows for the Web application to use heterogeneous resources of the clouds. In our tests, cheaper and smaller virtual machines were allocated to store only the contents that were involved in the flash-crowd event. 
	
	In both approaches, more eight virtual machines were hired during the flash crowd. However,  FCHP-ILS hired \textit{m3.medium} virtual machines with  enough storage capacity to keep only the contents involved in the flash crowd, which reduced the financial costs. By using Auto Scaling the total financial cost was \$$5.60$ for the Auto Scaling solution and was \$$4.08$ for our solution. The execution times were similar, around $5140$ seconds. Note that the proposed solutions, FCD and FCHP-ILS, present satisfactory results in real environments.
	

%	
	% We did not notice differences related to costs of transmitted data. 
	
	%Entretanto o custo de contratação de máquinas da solução do Auto Scaling foi de \$$3.04$, bem superior ao custo da solução FCHP-ILS, de \$$1.9$ -
	
	
	%ubiratam quero saber o total!!! Os custos de transferência de dados são os mesmos \$1.18.
	

	
	
		
	


